Anti-noise window: Subjective perception of active noise reduction and effect of informational masking

Reviving natural ventilation (NV) for urban sustainability presents challenges for indoor acoustic comfort. Active control and interference-based noise mitigation strategies, such as the use of loudspeakers, offer potential solutions to achieve acoustic comfort while maintaining NV. However, these approaches are not commonly integrated or evaluated from a perceptual standpoint. This study examines the perceptual and objective aspects of an active-noise-control (ANC)-based "anti-noise" window (ANW) and its integration with informational masking (IM) in a model bedroom. Forty participants assessed the ANW in a three-way interaction involving noise types (traffic, train, and aircraft), maskers (bird, water), and ANC (on, off). The evaluation focused on perceived annoyance (PAY; ISO/TS 15666), perceived affective quality (ISO/TS 12913-2), loudness (PLN), and included an open-ended qualitative assessment. Despite minimal objective reduction in decibel-based indicators and a slight increase in psychoacoustic sharpness, the ANW alone demonstrated significant reductions in PAY and PLN, as well as an improvement in ISO pleasantness across all noise types. The addition of maskers generally enhanced overall acoustic comfort, although water masking led to increased PLN. Furthermore, the combination of ANC with maskers showed interaction effects, with both maskers significantly reducing PAY compared to ANC alone.

==> tables/questionnaire.tex <==
\newcommand{\bigsq}{\scalebox{1.5}{$\square$}}

\begin{sffamily}
%\setcounter{table}{1}
\small
\noindent\textbf{\color{scolor}Table \thetable}\par%
\noindent{Pre-test assessment participant information questionnaire}
\label{tab:questionnaire}
%

\begin{tabularx}{\textwidth}{%
    >{\setlength\hsize{0.075\hsize}} X 
    >{\setlength\hsize{0.325\hsize}} X
    >{\setlength\hsize{0.575\hsize}} X
    >{\setlength\hsize{0.075\hsize}} X
    %*{5}{>{\centering\arraybackslash}X}%
}

\toprule
    Question Category
    & Instructions 
    & Specific Questions
    & Rating Scale \\

\midrule
    \multirow{21}{=}{Individual Noise Sensitivity (INS)}
    & \multirow{21}{=}{To what extent you disagree/agree with the following sentences?} 
    & `I wouldn’t mind living on a noisy street if the apartment I had was nice.'
    & \multirow{9}{=}{Strongly Disagree--Strongly Agree (5-point categorical)} \\ \cline{3-3}

    & & `No one should mind much if someone turns up his or her stereo full blast once in awhile.' 
    & \\ \cline{3-3}

    & & `I get used to most noises without much difficulty.’ 
    & \\ \cline{3-3}

    & & `It would matter to me if an apartment I was interested in renting were located across from a fire station.’ 
    & \\ \cline{3-3}

    & & `It wouldn’t bother me to hear the sounds of everyday living from neighbors (footsteps, running water, etc.).’  
    & \\ 

    & & `I’m good at concentrating no matter what is going on around me.' 
    & \\ \cline{3-3}

    & & `In a library, I don’t mind if people carry on a conversation if they do it quietly.’ 
    & \\ \cline{3-3}

    & & `I get mad at people who make noise that keeps me from falling asleep or getting work done.’ 
    & \\ \cline{3-3}

    & & `I wouldn’t mind living in an apartment with thin walls.’
    & \\ \cline{3-4}

    & & `I am more aware of noise than I used to be.’
    & \multirow{12}{=}{Strongly Agree--Strongly Disagree (5-point categorical)} \\ \cline{3-3}

    & & `At movies, whispering and crinkling candy wrappers disturb me.’
    & \\ \cline{3-3}

    & & `I am easily awakened by noise.’
    & \\ \cline{3-3}

    & & `If it’s noisy where I’m studying, I try to close the door or window or move someplace else.’
    & \\ \cline{3-3}

    & & `I get annoyed when my neighbors are noisy.’
    & \\ \cline{3-3}

    & & `Sometimes noises get on my nerves and get me irritated.’
    & \\ \cline{3-3}

    & & `Even music I normally like will bother me if I’m trying to concentrate.’
    & \\ \cline{3-3}

    & & `When I want to be alone, it disturbs me to hear outside noises.’
    & \\ \cline{3-3}

    & & `There are often times when I want complete silence.’
    & \\ \cline{3-3}

    & & `Motorcycles ought to be required to have bigger mufflers.’
    & \\ \cline{3-3}

    & & `I find it hard to relax in a place that’s noisy.’
    & \\ \cline{3-3}

    & & `I am sensitive to noise.’
    & \\ 
    
\midrule
    \multirow{10}{=}{Baseline Noise Annoyance (BAN)}
    & \multirow{5}{=}{Thinking about the last (12 months or so), when you are here at home, how much does noise from (noise source) bother, disturb or annoy you?} 
    & Road traffic 
    & \multirow{5}{=}{Not at all--Extremely (5-point categorical)} \\ \cline{3-3}

    & 
    & Aircraft  
    & \\ \cline{3-3}

    & 
    & MRT 
    & \\ \cline{3-3}

    & 
    & Construction Work (Work Site)
    & \\ \cline{3-3}

    & 
    & Construction Work (Renovations)
    & \\ \cline{3-3}

    & 
    & Any other noises (specify)
    & \\ \cline{2-4}
    
    & \multirow{5}{=}{ Thinking about the last (12 months or so), when you are here at home, how much does noise from (noise source) bother, disturb or annoy you?} 
    & Road traffic 
    & \multirow{5}{=}{Not at all--Extremely (0-to-100 numerical scale)} \\ \cline{3-3}

    & 
    & Aircraft  
    & \\ \cline{3-3}

    & 
    & MRT 
    & \\ \cline{3-3}

    & 
    & Construction Work (Work Site)
    & \\ \cline{3-3}

    & 
    & Construction Work (Renovations)
    & \\ \cline{3-3}

    & 
    & Any other noises (specify)
    & \\

\midrule
    \multirow{10}{=}{Perceived Stress Scale (PSS)}
    & \multirow{10}{=}{The questions in this scale ask you about your feelings and thoughts during the last month. In each case, you will be asked to indicate how often you felt or thought a certain way. Although some of the questions are similar, there are differences between them and you should treat each one as a separate question. The best approach is to answer each question fairly quickly. That is, don't try to count up the number of times you felt a particular way, but rather indicate the alternative that seems like a reasonable estimate. In the last month, how often have you... *} 
    & been upset because of something that happened unexpectedly? 
    & \multirow{10}{=}{Never--Very Often (5-point categorical)} \\ \cline{3-3}

    & & felt that you were unable to control the important things in your life
    & \\ \cline{3-3}

    & & felt nervous and "stressed"?
    & \\ \cline{3-3}

    & & felt confident about your ability to handle your personal problems?
    & \\ \cline{3-3}

    & & felt that things were going your way?
    & \\ \cline{3-3}

    & & found that you could not cope with all the things that you had to do?
    & \\ \cline{3-3}

    & & been able to control irritations in your life?
    & \\ \cline{3-3}

    & & felt that you were on top of things?
    & \\ \cline{3-3}

    & & been angered because of things that were outside of your control?
    & \\ \cline{3-3}

    & & felt difficulties were piling up so high that you could not overcome them?
    & \\ 

\midrule
    \multirow{5}{=}{WHO-5 Well Being Index (WHO-5)}
    & \multirow{5}{=}{For each of the statements below, which is the closest to how you have been feeling over the last two weeks?} 
    & I have felt cheerful and in good spirits. 
    & \multirow{5}{=}{At no time--All of the time (6-point categorical)} \\ \cline{3-3}

    & & I have felt calm and relaxed
    & \\ \cline{3-3}

    & & I have felt active and vigorous
    & \\ \cline{3-3}

    & & I woke up feeling fresh and rested.
    & \\ \cline{3-3}

    & & My daily life has been filled with things that interest me.
    & \\ 

\bottomrule
\end{tabularx}
\end{sffamily}
